Timeout Asynchronous Session Types: Safe Asynchronous Mixed-Choice For Timed Interactions

Mixed-choice has long been barred from models of asynchronous communication since it compromises the decidability of key properties of communicating finite-state machines. Session types inherit this restriction, which precludes them from fully modelling timeouts -- a core property of web and cloud services. To address this deficiency, we present (binary) Timeout Asynchronous Session Types (TOAST) as an extension to (binary) asynchronous timed session types, that permits mixed-choice. TOAST deploys timing constraints to regulate the use of mixed-choice so as to preserve communication safety. We provide a new behavioural semantics for TOAST which guarantees progress in the presence of mixed-choice. Building upon TOAST, we provide a calculus featuring process timers which is capable of modelling timeouts using a receive-after pattern, much like Erlang, and capture the correspondence with TOAST specifications via a type system for which we prove subject reduction.

==> figs/process_func_neq.tex <==
\begin{figure}[tb]
  \begin{pcalc}*
    \begin{array}[c]{@{}l@{\ }l@{\ }l@{}}
      \NEQ & = & \begin{cases}
                   \{\q\}
                    & \text{if\ } \P=\pq:\h\land\h\neq\emptyset
                   \\[0.5ex]
                   \NEQ{\Q}\setminus\{\p,\q\}
                    & \text{if\ } \P=\Scope{\pq}{\Q}
                   \\[0.5ex]
                   \NEQ{\Q}
                    & \text{if\ } \P=\Def{\Rec*{V;T;R}=\P'}:{\Q}
                   \\[0.5ex]
                   \NEQ{\P'}\cup\NEQ{\Q}
                    & \text{if\ } \P=\P'\mid\Q
                   \\[0.5ex]
                   \emptyset
                    & \text{otherwise}
                 \end{cases}
    \end{array}
  \end{pcalc}
  \caption{Definition of \PCalc{\NEQ}.}\label{fig:func_neq}
\end{figure}



==> figs/process_func_wait.tex <==
\begin{figure}[tb]
  \begin{pcalc}*
    \begin{array}[c]{@{}l@{\ }l@{\ }l@{}}
      \Wait & = & \begin{cases}
                    \{\p\}
                     & \text{if\ } \P \in \begin{array}[t]\{{@{}l@{}}\}
                                \On{\p}\Recv^{\e}{\l}[\v]:{\P}_i~\After{\n}:{\Q},%
                                \\[0.25ex]
                                \On{\p}\Recv^{\e}{\l}[\v]:{\P}_i
                              \end{array}
                    \\[0.5ex]
                    \Wait{\Q}\setminus\{\p,\q\}
                     & \text{if\ } \P=\Scope{\pq}{\Q}
                    \\[0.5ex]
                    \Wait{\Q}
                     & \text{if\ } \P=\Def{\Rec*{V;T;R}=\P'}:{\Q}
                    \\[0.5ex]
                    \Wait{\P'}\cup\Wait{\Q}
                     & \text{if\ } \P=\P'\mid\Q
                    \\[0.5ex]
                    \emptyset
                     & \text{otherwise}
                  \end{cases}
    \end{array}
  \end{pcalc}
  \caption{Definition of \PCalc{\Wait}.}\label{fig:func_wait}
\end{figure}



==> figs/process_func_wf.tex <==
\begin{defi}[Well-formed Process]\label{def:func_wf}
  The function \WF{\P}\ is defined inductively as:
  \small\[
    \begin{array}[t]{@{}l@{}}
      %
      \WF{\P}
      = \begin{cases}
          %
          \True                                                  &
          \text{if\ }\P\in\begin{array}[c]\{{@{}l@{}}\}
                          %
                          \Term,
                          % \\
                          ~\Rec,
                          % \\
                          ~{\qp:\h}
                          %
                        \end{array}
          %
          \\[\ArrayExtraTallLineSpacing]
          \WF{\P'} \land \FQ{\P'}=\{\pq,\qp\}                    &
          \text{if\ }\P=\Scope{\pq}{\P'}
          %
          \\[\ArrayTallLineSpacing]
          \WF{\P'} \land \FQ{\P'}=\emptyset                      &
          \text{if\ }\P\in\begin{array}[c]\{{@{}l@{}}\}
                          %
                          \On{\p}\Send{\l}[\v]{\P'},
                          ~\Set{x}.\P',
                          % ~\Scope{\pq}{\P'}, % !<- 
                          % ~\Def{\Rec*{\vec{v};\vec{r}}=\P}:{\P'}
                          \\
                          \Delay{\Duration}.\P',
                          ~\Delay{\t}.\P'
                          %
                        \end{array}
          %
          \\[\ArrayExtraTallLineSpacing]
          \bigwedge_{i\in I} \WF{\P_i} \land \FQ{\P_i}=\emptyset &
          \text{if\ }\P =
          \On{\p}\Recv^{\e}{\l}[\v]:{\P}_i
          %
          \\[\ArrayExtraTallLineSpacing]
          \WF{\P'} \land \WF{\Q}                                 &
          \begin{array}[t]{@{}l@{}}
          \text{if\ }\P\in\begin{array}[c]\{{@{}l@{}}\}
                            %
                            {\P'\mid\Q},
                            ~\If*{\Cond}~\Then{\P'}~\Else{\Q}
                            % ~\If{\Cond}\Then{\P'}~\Else{\Q}
                            \\
                            ~\Def{\Rec*{\vec{v};\vec{r}}=\P'}:{\Q}
                            %
                          \end{array}
        \end{array}
          %
          \\[\ArrayExtraTallLineSpacing]
          \WF{\On{\p}\Recv^{\e}{\l}[\v]:{\P}_i} \land \WF{\Q}    &
          \text{if\ }\P=\after{\p}{\e}{\l}{\v}{\P}{\Q}
          %
        \end{cases}
      %
    \end{array}
  \]
  %
\end{defi}



==> macros/theory/liveness.tex <==

\NewDocumentCommand{\SL}{t+ G{\PrcCalcP}}{\WrapMathMode{\mathtt{SL}\IfBooleanT{#1}{^{+}}(#2)}}

\NewDocumentCommand{\NZ}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{NZ}(#1)}}

\NewDocumentCommand{\TO}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{TO}(#1)}}

\NewDocumentCommand{\Roles}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{R}(#1)}}

\NewDocumentCommand{\Sending}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{Send}(#1)}}
\NewDocumentCommand{\Receiving}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{Recv}(#1)}}
\NewDocumentCommand{\Inter}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{Inter}(#1)}}
\NewDocumentCommand{\Tail}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{Tail}(#1)}}


\NewDocumentCommand{\PRecv}{e_ t' G{1}}{\WrapMathMode{%
      \IfValueTF{#1}{%
         {P}\IfBooleanT{#2}{\RepeatChar{#3}{'}}_{#1}^{\RecvSym*}%
      }{%
         {P}\IfBooleanT{#2}{\RepeatChar{#3}{'}}^{\RecvSym*}%
      }%
   }%
}

\NewDocumentCommand{\QRecv}{e_ t' G{1}}{\WrapMathMode{%
      \IfValueTF{#1}{%
         {Q}\IfBooleanT{#2}{\RepeatChar{#3}{'}}_{#1}^{\RecvSym*}%
      }{%
         {Q}\IfBooleanT{#2}{\RepeatChar{#3}{'}}^{\RecvSym*}%
      }%
   }%
}


\RenewDocumentCommand{\PrcCalcP}{s e_ t' G{1}}{%
\PrcCalcPrc{\IfBooleanTF{#1}{\hat{P}}{P}}_{#2}'{\IfBooleanTF{#3}{#4}{0}}%
}

\RenewDocumentCommand{\PrcCalcQ}{s e_ t' G{1}}{%
\PrcCalcPrc{\IfBooleanTF{#1}{\hat{Q}}{Q}}_{#2}'{\IfBooleanTF{#3}{#4}{0}}%
}


% context
%% #1 : s* : surface-level context (?)
%% #2 : t- : instantaneous reduction context (?)
%% #3 : t~ : time-passing reduction context (?)
%% #4 : [] : content of context [ ]
%% #5 : e_ : subscript _
%% #6 : t' : prime '
%% #7 : {} : (optional) number of '
%% # :  : 
%% # :  : 
\NewDocumentCommand{\Ct}{s t- t~ o e_ t' G{1}}{\WrapMathMode{%\mathbb{C}%
   {\mathbb{C}%
   \IfBooleanT{#1}{^{\mathtt{\ast}}}%
   \IfValueTF{#5}{_{#5}}{\IfBooleanT{#3}{_{\t}}}%
   \IfBooleanF{#1}{% * reduction context
      \IfBooleanT{#2}{^{\scriptscriptstyle \Reduce-}}%
      \IfBooleanT{#3}{^{\scriptscriptstyle \Reduce~}}%
      % \IfBooleanF{#2}{\IfBooleanF{#3}{^{\scriptscriptstyle \rightarrow}}}%
   }}%
   \IfBooleanT{#6}{\RepeatChar{#7}{'}}%
   % * context content
   \IfValueT{#4}{[#4]}%
}}


\NewDocumentCommand{\SSP}{s G{\PrcCalcP}}{\WrapMathMode{\mathtt{ssp}\IfBooleanF{#1}{(#2)}}}
\NewDocumentCommand{\ISP}{s G{\PrcCalcP}}{\WrapMathMode{\mathtt{isp}\IfBooleanF{#1}{(#2)}}}



%% predicates
\NewDocumentCommand{\PredTo}{s e^ G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{to}\IfValueT{#2}{^{#2}}(#3,#4)}}

\NewDocumentCommand{\PredIn}{s e^ G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{in\IfBooleanT{#1}{\ast}}\IfValueT{#2}{^{#2}}(#3,#4)}}

\NewDocumentCommand{\PredOut}{G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{out}(#1,#2)}}
% \NewDocumentCommand{\PredSync}{G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{sync}(#1,#2)}}
% \NewDocumentCommand{\PredWait}{G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{wait}(#1,#2)}}

\NewDocumentCommand{\PredEmpty}{G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{empty}(#1,#2)}}
\NewDocumentCommand{\PredMail}{G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{mail}(#1,#2)}}

% \NewDocumentCommand{\PredRecv}{G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{recv}(#1,#2)}}

% \NewDocumentCommand{\PredScry}{G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{scry}(#1,#2)}}

\NewDocumentCommand{\PredWait}{s G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{wait}(\IfBooleanTF{#1}{#2}{#2,#3})}}

\NewDocumentCommand{\PredRecv}{s G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{recv}(\IfBooleanTF{#1}{#2}{#2,#3})}}

\NewDocumentCommand{\PredScry}{s G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{scry}(\IfBooleanTF{#1}{#2}{#2,#3})}}

\NewDocumentCommand{\PredSync}{s G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{sync}(\IfBooleanTF{#1}{#2}{#2,#3})}}

\NewDocumentCommand{\PredLive}{s G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{live}(\IfBooleanTF{#1}{#2}{#2,#3})}}

\NewDocumentCommand{\PredStuck}{s G{\PrcCalcp} G{\PrcCalcP}}{\WrapMathMode{\mathtt{stuck}(\IfBooleanTF{#1}{#2}{#2,#3})}}

\NewDocumentCommand{\PredGood}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{good}(#1)}}

\NewDocumentCommand{\PredDead}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{dead}(#1)}}

\NewDocumentCommand{\PredLocked}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{locked}(#1)}}

\NewDocumentCommand{\PredZeno}{G{\PrcCalcP}}{\WrapMathMode{\mathtt{zeno}(#1)}}

\NewDocumentCommand{\PredQueue}{t0 G{\PrcCalcP}}{\WrapMathMode{\mathtt{queue}\IfBooleanT{#1}{^{\emptyset}}(#2)}}


\NewDocumentCommand{\bn}{s G{\PrcCalcP}}{\WrapMathMode{\mathtt{bn}(\IfBooleanTF{#1}{\Ct*}{#2})}}
\NewDocumentCommand{\fn}{s G{\PrcCalcP}}{\WrapMathMode{\mathtt{fn}(\IfBooleanTF{#1}{\Ct*}{#2})}}


==> macros/tools.tex <==

% ~ better not for xrightarrows
% https://tex.stackexchange.com/questions/124096/how-do-i-create-a-negated-arrow-on-xrightarrow
\makeatletter
\def\slashedarrowfill@#1#2#3#4#5{%
    $\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
        \relax#5#1\mkern-7mu%
        \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
        \mathclap{#3}\mathclap{#2}%
        \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
        \mkern-7mu#4$%
}
\def\rightslashedarrowfill@{%
    \slashedarrowfill@\relbar\relbar{\raisebox{1pt}[0pt]{$\scriptscriptstyle\diagup$}}\rightarrow}
% % lowering arrow
% \newcommand\xnrightarrow[2][]{%
%     \raisebox{-1pt}[10.5pt]{$\ext@arrow 0055\rightslashedarrowfill@{#1}{#2}$}}
% \newcommand\xrightarrow[2][]{%
%     \raisebox{-1pt}[10.5pt]{$\ext@arrow 0055\rightarrowfill@{#1}{#2}$}}
% lowering arrow
\newcommand\xnrightarrow[2][]{%
    \raisebox{-1pt}[12.5pt]{$\ext@arrow 0055\rightslashedarrowfill@{#1}{#2}$}}
\newcommand\xrightarrow[2][]{%
    \raisebox{-1pt}[12.5pt]{$\ext@arrow 0055\rightarrowfill@{#1}{#2}$}}
% redefined 
\makeatother

% ~ wraps in math mode if not in math mode
% https://tex.stackexchange.com/questions/46492/newcommand-how-to-determine-if-in-math-mode-and-then-include
% #1 : s* : escape math-mode if in math-mode?
\DeclareDocumentCommand{\WrapMathMode}{s m}{%
    \relax\ifmmode% in math-mode
        \IfBooleanTF{#1}{$#2$}{#2}% escape if s*
    \else% outside math-mode
        \IfBooleanTF{#1}{#2}{$#2$}% wrap if no s*
    \fi%
}

% ~ substitution/renaming notation
\NewDocumentCommand{\Subst}{m m}{\WrapMathMode{%
        \left[{\sfrac{#1}{#2}}\right]%
    }%
}

% ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ 
% ~ xparse list processors 
% ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~

% ~ CSV list separated by line break for array
\NewDocumentCommand{\CSVListToArrayLines}{>{\SplitList{,}}m}{%
    \ProcessList{#1}{\HeadCSVListToArrayLines}
}
\NewDocumentCommand{\HeadCSVListToArrayLines}{m}{%
    \rule{0pt}{1.5ex}{#1}%
    \let\HeadCSVListToArrayLines\TailCSVListToArrayLines%
}
\NewDocumentCommand{\TailCSVListToArrayLines}{m}{%
    \\[0.5ex]%
    \rule{0pt}{1.5ex}{#1}%
    \let\HeadCSVListToArrayLines\TailCSVListToArrayLines%
}

% ~ CSV list spaced without commas
\NewDocumentCommand{\CSVListToSpacedLabels}{>{\SplitList{,}}m}{%
    \ProcessList{#1}{\HeadCSVListToSpacedLabels}
}
\NewDocumentCommand{\HeadCSVListToSpacedLabels}{m}{%
    \rule{0pt}{1.5ex}{#1}%
    \let\HeadCSVListToSpacedLabels\TailCSVListToSpacedLabels%
}
\NewDocumentCommand{\TailCSVListToSpacedLabels}{m}{%
~{\rule{0pt}{1.5ex}{#1}}%
\let\HeadCSVListToSpacedLabels\TailCSVListToSpacedLabels%
}

% ~ Semicolon-SV list separated ; for recursive process triple
\NewDocumentCommand{\ScSVListToRecPrc}{>{\SplitList{;}}m}{%
    \ProcessList{#1}{\HeadScSVListToRecPrc}
    % \IfValueTF{#2}{%
    %     \ProcessList{#1}{\HeadScSVListToRecPrc}%
    % }{%
    %     \ProcessList{#1}{\HeadScSVListToRecPrc}%
    % }%
}
\NewDocumentCommand{\HeadScSVListToRecPrc}{>{\SplitArgument{1}{:}}m}{%
    \rule{0pt}{1.5ex}{\FormatRecVarStyle #1 }%
    \let\HeadScSVListToRecPrc\TailScSVListToRecPrc%
}
\NewDocumentCommand{\TailScSVListToRecPrc}{>{\SplitArgument{1}{:}}m}{%
    ;%
    \rule{0pt}{1.5ex}{\FormatRecVarStyle #1 }%
    \let\HeadScSVListToRecPrc\TailScSVListToRecPrc%
}

% ~ Semicolon-SV list separated ; for recursive definition triple
\NewDocumentCommand{\ScSVListToRecCheck}{>{\SplitList{;}}m}{%
    \ProcessList{#1}{\HeadScSVListToRecCheck}
}
\NewDocumentCommand{\HeadScSVListToRecCheck}{m}{%
    \rule{0pt}{1.5ex}{\FormatRecCheckStyle{#1}}%
    \let\HeadScSVListToRecCheck\TailScSVListToRecCheck%
}
\NewDocumentCommand{\TailScSVListToRecCheck}{m}{%
    ;%
    \rule{0pt}{1.5ex}{\FormatRecCheckStyle{#1}}%
    \let\HeadScSVListToRecCheck\TailScSVListToRecCheck%
}


% ~ CSV list separated , for recursive process triple
\NewDocumentCommand{\CSVListToRecPrc}{>{\SplitList{,}}m}{%
    \ProcessList{#1}{\HeadCSVListToRecPrc}
}
\NewDocumentCommand{\HeadCSVListToRecPrc}{m}{%
    \rule{0pt}{1.5ex}{\FormatRecVarStyle{#1}}%
    \let\HeadCSVListToRecPrc\TailCSVListToRecPrc%
}
\NewDocumentCommand{\TailCSVListToRecPrc}{m}{%
    ,%
    \rule{0pt}{1.5ex}{\FormatRecVarStyle{#1}}%
    \let\HeadCSVListToRecPrc\TailCSVListToRecPrc%
}

% ~ CSV list separated , for recursive definition triple
\NewDocumentCommand{\CSVListToRecCheck}{>{\SplitList{,}}m}{%
    \ProcessList{#1}{\HeadCSVListToRecCheck}
}
\NewDocumentCommand{\HeadCSVListToRecCheck}{m}{%
    \rule{0pt}{1.5ex}{\FormatRecCheckStyle{#1}}%
    \let\HeadCSVListToRecCheck\TailCSVListToRecCheck%
}
\NewDocumentCommand{\TailCSVListToRecCheck}{m}{%
    ,%
    \rule{0pt}{1.5ex}{\FormatRecCheckStyle{#1}}%
    \let\HeadCSVListToRecCheck\TailCSVListToRecCheck%
}


% ~ repeat character n times
% https://tex.stackexchange.com/questions/300207/repeat-characters-n-times
\makeatletter%
\newcommand{\RepeatChar}[2]{%
    \begingroup%
    \lccode`m=`#2\relax%
    \lowercase\expandafter{\romannumeral#1000}%%
    \endgroup%
    % \negthinspace% to avoid outer ',',' spacing errors? 
}%
\makeatother%

